Compact Real-time Radiance Fields with Neural Codebook

Reconstructing neural radiance fields with explicit volumetric representations, demonstrated by Plenoxels, has shown remarkable advantages on training and rendering efficiency, while grid-based representations typically induce considerable overhead for storage and transmission. In this work, we present a simple and effective framework for pursuing compact radiance fields from the perspective of compression methodology. By exploiting intrinsic properties exhibiting in grid models, a non-uniform compression stem is developed to significantly reduce model complexity and a novel parameterized module, named Neural Codebook, is introduced for better encoding high-frequency details specific to per-scene models via a fast optimization. Our approach can achieve over 40 $\times$ reduction on grid model storage with competitive rendering quality. In addition, the method can achieve real-time rendering speed with 180 fps, realizing significant advantage on storage cost compared to real-time rendering methods.

==> prelim.tex <==

\section{Preliminary}
Neural Radiance fields (NeRF) \cite{NeRF} are formulated as learning a continuous
mapping function between a 5D coordinate, e.g., 3D spatial position $\mathbf{x} \in \mathbb{R}^3$ with a view direction $\mathbf{d} \in \mathbb{R}^2$
%(represented as a Cartesian unit vector)
, and its
corresponding volume density $\sigma \in \mathbb{R}$ and view-dependent color $\mathbf{c} \in \mathbb{R}^3$. The mapping function is instantiated by multilayer perceptron (MLP) networks $f_{m}: (\mathbf{x}, \mathbf{d}) \mapsto (\mathbf{c}, \sigma)$, equipped with nonlinear activations (e.g., ReLU). The radiance field of a scene is reconstructed through the use of volume rendering techniques \cite{OpticalModel}. The color $\hat{C}(\mathbf{r})$ at the position $\mathbf{x}$ is rendered by casting the ray $\mathbf{r}$ from the camera center through it, sampling $N$ points along the ray between the predefined near and far planes, and querying their colors and densities ${\mathbf{c}_i, \sigma_i}$ through the network $f_{m}$. Finally, a single color is produced by accumulating them by using the following volume rendering quadrature formula,
\begin{equation}\label{eq:render} 
    \widehat{C}(\mathbf{r}) = \sum_{i=1}^N T_i\cdot \alpha_i \cdot \mathbf{c}_i,
\end{equation}
\begin{equation}\label{eq:alpha_t}
    \alpha_i = 1 - \exp(-\sigma_i \delta_i),\quad T_i = \prod_{j=1}^{i-1} (1 - \alpha_j),
\end{equation}
forming a weighted summation on sampling point colors. $\alpha_i$ denotes the ray termination probability, $T_i$ represents the accumulated transmittance when reaching at $i$, and $\delta_i$ denotes the distance to adjacent points. An NeRF network is trained by minimizing a photometric loss of a batch of rays between their predicted colors and the corresponding ground-truths in the training images. By virtue of an implicit formulation, these methods are capable of representing 3D scenes with impressive quality and flexibility. As a large number of points are sampled for each ray and each point needs to be fed into a single large network for computation, implicit methods typically suffer from considerable computational complexity during training and rendering stage. 

In contrast, explicit methods, e.g., Plenoxels \cite{yu2021plenoxels}, use a volume grid based representations. Formally, the volume density and the features inducing view-variant colors are respectively represented as $\mathbf{V}_{\sigma} \in \mathbb{R}^{H\times W\times K}$ and $\mathbf{V}_{c} \in \mathbb{R}^{H\times W\times K\times C}$. Here $H$, $W$ and $K$ correspond to the spatial resolutions. Particularly, color features are produced by using a set of spherical harmonics (SH) in which the coefficients act as features (the dimension is $C$) to be optimized and can be inferred directly given the target viewing direction, allowing much higher efficiency on training and inference compared to the implicit representation methods.  
